A Language Support for Exhaustive Fault-Injection in Message-Passing System Models

This paper presents an approach towards specifying and verifying adaptive distributed systems. We here take fault-handling as an example of adaptive behavior and propose a modeling language Sandal for describing fault-prone message-passing systems. One of the unique mechanisms of the language is a linguistic support for abstracting typical faults such as unexpected termination of processes and random loss of messages. The Sandal compiler translates a model into a set of NuSMV modules. During the compilation process, faults specified in the model will be woven into the output. One can thus enjoy full-automatic exhaustive fault-injection without writing faulty behaviors explicitly. We demonstrate the advantage of the language by verifying a model of the two-phase commit protocol under faulty environment.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{M. M. Bersani, D. Bresolin, L. Ferrucci and M. Mazzara (Eds.): \\
First Workshop on Logics and MODel-checking for self-* systems (MOD*)\\
EPTCS 168, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.168.4}{10.4204/EPTCS.168.4}}

